Coded Caching over Multicast Routing Networks

The coded caching scheme originally proposed by Maddah-Ali and Niesen (MAN) transmits coded multicast messages from a server to users equipped with caches via a capacitated shared-link and was shown to be information theoretically optimal within a constant multiplicative factor. This work extends the MAN scheme to a class of two-hop wired-wireless networks including one server connected via fronthaul links to a layer of $H$ helper nodes (access points/base stations), which in turns communicate via a wireless access network to $K$ users, each equipped with its own cache. Two variants are considered, which differ in the modeling of the access segment. Both models should be regarded as abstractions at the network layer for physical scenarios such as local area networks and cellular networks, spatially distributed over a certain coverage area. The key focus of our approach consists of routing MAN-type multicast messages through the network and formulating the optimal routing scheme as an optimization problem that can be solved exactly or for which we give powerful heuristic algorithms. Our approach solves at once many of the open practical problems identified as stumbling blocks for the application of coded caching in practical scenarios, namely: asynchronous streaming sessions, finite file size, scalability of the scheme to large and spatially distributed networks, user mobility and random activity (users joining and leaving the system at arbitrary times), decentralized prefetching of the cache contents, end-to-end encryption of HTTPS requests, which renders the helper nodes oblivious of the user demands.

==> symbols.tex <==
%symbols.tex     symbols for book using Springer style files.
\usepackage{mathbbol}


%%%%%%%%%%%%%%%%%%%%%%
\def\mindex#1{\index{#1}}

\def\sindex#1{\index{#1}}

%\typeout{REMOVE SINDEX AND MINDEX AT END}
%\typeout{CHECK NOTES IN SPRINGER3}


\def\slPi{{\mit\Pi}}

\def\contains{\supset}


% Colored Texts
%\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% qed
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\sq\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\sq
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi\medskip}



%%%%%%%%%%%%%%%%%%FOR DEFINITIONS


\long\def\defbox#1{\framebox[.9\hsize][c]{\parbox{.85\hsize}{%
\parindent=0pt
\baselineskip=12pt plus .1pt      % STYLE
\parskip=6pt plus 1.5pt minus 1pt % CHANGES
 #1}}}


%% Much improved beginbox:

\long\def\beginbox#1\endbox{\subsection*{}%
\hbox{\hspace{.05\hsize}\defbox{\medskip#1\bigskip}}%
\subsection*{}}

\def\endbox{}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MATH OPERATORS

\def\transpose{{\hbox{\it\tiny T}}}

\def\diag{{\text{diag}}}

\def\mm{\phantom{-}}

\def\wkarrow{\buildrel{\rm w}\over\longrightarrow}
\def\vgarrow{\buildrel{\rm v}\over\longrightarrow}
\def\tvlimit#1{\buildrel{\scriptscriptstyle #1}\over\Longrightarrow}
\def\darrow{\buildrel{\rm d}\over\longrightarrow}

\def\goes#1{\buildrel{#1}\over\longrightarrow}
\def\wiggles#1{\buildrel{#1}\over\leadsto}


\def\tr{\mathsf{Tr}}

\def\rank{{\rm rank\,}}
\def\deg{\hbox{\rm deg\thinspace}}
\def\sign{{\rm sign}}
\def\supp{{\rm supp\,}}


\newsavebox{\junk}
\savebox{\junk}[1.6mm]{\hbox{$|\!|\!|$}}
\def\lll{{\usebox{\junk}}}


\def\det{{\mathop{\rm det}}}
\def\limsup{\mathop{\rm lim\ sup}}
\def\liminf{\mathop{\rm lim\ inf}}
\def\argmin{\mathop{\rm arg\, min}}

\def\argmax{\mathop{\rm arg\, max}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPACES



\def\A{{\sf A}}
\def\K{{\sf K}}
\def\U{{\sf U}}
\def\V{{\sf V}}
\def\W{{\sf W}}

\def\state{{\sf X}}
\def\ystate{{\sf Y}}

\def\zstate{{\sf Z}}


%\def\smallsfX{{\hbox{\scriptsize\sf X}}}
%\def\sfX{{\hbox{\sf X}}}
%\def\state{{\mathchoice\sfX\sfX\smallsfX\smallsfX}}


%\def\smallsfY{{\hbox{\scriptsize\sf Y}}}
%\def\sfY{{\hbox{\sf Y}}}
%\def\ystate{{\mathchoice\sfY\sfY\smallsfY\smallsfY}}

\def\by{\clB(\ystate)}

\def\tinyplus{\vbox{\hrule width 3pt depth -1.5pt height 1.9pt
      \vskip -1.5pt
      \hbox{\hskip 1.3pt\vrule height 3pt depth 0pt width .4pt}}}


\def\xz{{\sf X^{\rm z}}}
\def\bxz{{\cal B}(\state^\hbox{\rm\tiny z})}
\def\xzplus{{\sf X^{{\rm z}_{ \tinyplus}}}}
\def\xbxm{({\sf X},{\cal B}({\bf X}),{\bf m})}
\def\bx{{{\cal B}(\state)}}
\def\bxzplus{{\cal B}(\state^{{\rm z}_{\tinyplus}} )} \def\bxplus{{\clB^+(\state)}}


\newcommand{\field}[1]{\mathbb{#1}}



\def\posRe{\field{R}_+}
\def\Re{\field{R}}

\def\A{\field{A}}


\def\One{\mbox{\rm{\large{1}}}}
\def\Zero{\mbox{\rm{\large{0}}}}


\def\ind{\field{I}}


\def\TT{\field{T}}
\def\ZZ{\field{Z}}


\def\intgr{\field{Z}}

\def\nat{\field{Z}_+}


\def\rat{\field{Q}}

\def\Co{\field{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CHECKED CHARACTERS



\def\cclF{{\check{\clF}}}
\def\catom{{\check{\atom}}}
\def\cExpect{\check{\Expect}}
\def\cPhi{\check{\Phi}}
\def\cbfPhi{\check{\bfPhi}}
\def\cProb{\check{\Prob}}
\def\cProbsub{\cProb\!}
\def\cPhi{\check{\Phi}}

\def\cpi{\check{\pi}}
\def\cA{\check{A}}

\def\cG{{\check{G}}}

\def\cP{{\check{P}}}
\def\cbxplus{{\cal B}^+(\cstate)}
\def\cstate{{\check{\state}}}
\def\bcx{\clB(\cstate)}

\def\LPhi{\bfPhi^{\Lambda}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BF PREFIXES

\def\bA{{\mathbb A}}
\def\bB{{\mathbb B}}
\def\bC{{\mathbb C}}
\def\bD{{\mathbb D}}
\def\bE{{\mathbb E}}
\def\bF{{\mathbb F}}
\def\bG{{\mathbb G}}
\def\bH{{\mathbb H}}
\def\bI{{\mathbb I}}
\def\bJ{{\mathbb J}}
\def\bK{{\mathbb K}}
\def\bL{{\mathbb L}}
\def\bM{{\mathbb M}}
\def\bN{{\mathbb N}}
\def\bO{{\mathbb O}}
\def\bP{{\mathbb P}}
\def\bQ{{\mathbb Q}}
\def\bR{{\mathbb R}}
\def\bS{{\mathbb S}}
\def\bT{{\mathbb T}}
\def\bU{{\mathbb U}}
\def\bV{{\mathbb V}}
\def\bW{{\mathbb W}}
\def\bX{{\mathbb X}}
\def\bY{{\mathbb Y}}
\def\bZ{{\mathbb Z}}






\def\bba{{\mathbb a}}
\def\bbb{{\mathbb b}}
\def\bbc{{\mathbb c}}
\def\bbd{{\mathbb d}}
\def\bbe{{\mathbb e}}
\def\bbf{{\mathbb f}}
\def\bbg{{\mathbb g}}
\def\bbh{{\mathbb h}}
\def\bbi{{\mathbb i}}
\def\bbj{{\mathbb j}}
\def\bbk{{\mathbb k}}
\def\bbl{{\mathbb l}}
\def\bbm{{\mathbb m}}
\def\bbn{{\mathbb n}}
\def\bbo{{\mathbb o}}
\def\bbp{{\mathbb p}}
\def\bbq{{\mathbb q}}
\def\bbr{{\mathbb r}}
\def\bbs{{\mathbb s}}
\def\bbt{{\mathbb t}}
\def\bbu{{\mathbb u}}
\def\bbv{{\mathbb v}}
\def\bbw{{\mathbb w}}
\def\bbx{{\mathbb x}}
\def\bby{{\mathbb y}}
\def\bbz{{\mathbb z}}



%\def\ba{{\mathbb a}}
%\def\bb{{\mathbb b}}
%\def\bc{{\mathbb c}}
%\def\bd{{\mathbb d}}
%\def\be{{\mathbb e}}
%\def\bf{{\mathbb f}}
%\def\bg{{\mathbb g}}
%\def\bh{{\mathbb h}}
%\def\bi{{\mathbb i}}
%\def\bj{{\mathbb j}}
%\def\bk{{\mathbb k}}
%\def\bl{{\mathbb l}}
%\def\bm{{\mathbb m}}
%\def\bn{{\mathbb n}}
%\def\bo{{\mathbb o}}
%\def\bp{{\mathbb p}}
%\def\bq{{\mathbb q}}
%\def\br{{\mathbb r}}
%\def\bs{{\mathbb s}}
%\def\bt{{\mathbb t}}
%\def\bu{{\mathbb u}}
%\def\bv{{\mathbb v}}
%\def\bw{{\mathbb w}}
%\def\bx{{\mathbb x}}
%\def\by{{\mathbb y}}
%\def\bz{{\mathbb z}}











\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfC{{\bf C}}
\def\bfD{{\bf D}}
\def\bfE{{\bf E}}
\def\bfF{{\bf F}}
\def\bfG{{\bf G}}
\def\bfH{{\bf H}}
\def\bfI{{\bf I}}
\def\bfJ{{\bf J}}
\def\bfK{{\bf K}}
\def\bfL{{\bf L}}
\def\bfM{{\bf M}}
\def\bfN{{\bf N}}
\def\bfO{{\bf O}}
\def\bfP{{\bf P}}
\def\bfQ{{\bf Q}}
\def\bfR{{\bf R}}
\def\bfS{{\bf S}}
\def\bfT{{\bf T}}
\def\bfU{{\bf U}}
\def\bfV{{\bf V}}
\def\bfW{{\bf W}}
\def\bfX{{\bf X}}
\def\bfY{{\bf Y}}
\def\bfZ{{\bf Z}}

\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfc{{\bf c}}
\def\bfd{{\bf d}}
\def\bfe{{\bf e}}
\def\bff{{\bf f}}
\def\bfg{{\bf g}}
\def\bfh{{\bf h}}
\def\bfi{{\bf i}}
\def\bfj{{\bf j}}
\def\bfk{{\bf k}}
\def\bfl{{\bf l}}
\def\bfm{{\bf m}}
\def\bfn{{\bf n}}
\def\bfo{{\bf o}}
\def\bfp{{\bf p}}
\def\bfq{{\bf q}}
\def\bfr{{\bf r}}
\def\bfs{{\bf s}}
\def\bft{{\bf t}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfw{{\bf w}}
\def\bfx{{\bf x}}
\def\bfy{{\bf y}}
\def\bfz{{\bf z}}


%%

\def\frkA{{\mathfrak{A}}}
\def\frkB{{\mathfrak{B}}}
\def\frkC{{\mathfrak{C}}}
\def\frkD{{\mathfrak{D}}}
\def\frkE{{\mathfrak{E}}}
\def\frkF{{\mathfrak{F}}}
\def\frkG{{\mathfrak{G}}}
\def\frkH{{\mathfrak{H}}}
\def\frkI{{\mathfrak{I}}}
\def\frkJ{{\mathfrak{J}}}
\def\frkK{{\mathfrak{K}}}
\def\frkL{{\mathfrak{L}}}
\def\frkM{{\mathfrak{M}}}
\def\frkN{{\mathfrak{N}}}
\def\frkO{{\mathfrak{O}}}
\def\frkP{{\mathfrak{P}}}
\def\frkQ{{\mathfrak{Q}}}
\def\frkR{{\mathfrak{R}}}
\def\frkS{{\mathfrak{S}}}
\def\frkT{{\mathfrak{T}}}
\def\frkU{{\mathfrak{U}}}
\def\frkV{{\mathfrak{V}}}
\def\frkW{{\mathfrak{W}}}
\def\frkX{{\mathfrak{X}}}
\def\frkY{{\mathfrak{Y}}}
\def\frkZ{{\mathfrak{Z}}}

\def\frka{{\mathfrak a}}
\def\frkb{{\mathfrak b}}
\def\frkc{{\mathfrak c}}
\def\frkd{{\mathfrak d}}
\def\frke{{\mathfrak e}}
\def\frkf{{\mathfrak f}}
\def\frkg{{\mathfrak g}}
\def\frkh{{\mathfrak h}}
\def\frki{{\mathfrak i}}
\def\frkj{{\mathfrak j}}
\def\frkk{{\mathfrak k}}
\def\frkl{{\mathfrak l}}
\def\frkm{{\mathfrak m}}
\def\frkn{{\mathfrak n}}
\def\frko{{\mathfrak o}}
\def\frkp{{\mathfrak p}}
\def\frkq{{\mathfrak q}}
\def\frkr{{\mathfrak r}}
\def\frks{{\mathfrak s}}
\def\frkt{{\mathfrak t}}
\def\frku{{\mathfrak u}}
\def\frkv{{\mathfrak v}}
\def\frkw{{\mathfrak w}}
\def\frkx{{\mathfrak x}}
\def\frky{{\mathfrak y}}
\def\frkz{{\mathfrak z}}


%%%

%% scr fonts




\def\scrA{{\mathscr{A}}}
\def\scrB{{\mathscr{B}}}
\def\scrC{{\mathscr{C}}}
\def\scrD{{\mathscr{D}}}
\def\scrE{{\mathscr{E}}}
\def\scrF{{\mathscr{F}}}
\def\scrG{{\mathscr{G}}}
\def\scrH{{\mathscr{H}}}
\def\scrI{{\mathscr{I}}}
\def\scrJ{{\mathscr{J}}}
\def\scrK{{\mathscr{K}}}
\def\scrL{{\mathscr{L}}}
\def\scrM{{\mathscr{M}}}
\def\scrN{{\mathscr{N}}}
\def\scrO{{\mathscr{O}}}
\def\scrP{{\mathscr{P}}}
\def\scrQ{{\mathscr{Q}}}
\def\scrR{{\mathscr{R}}}
\def\scrS{{\mathscr{S}}}
\def\scrT{{\mathscr{T}}}
\def\scrU{{\mathscr{U}}}
\def\scrV{{\mathscr{V}}}
\def\scrW{{\mathscr{W}}}
\def\scrX{{\mathscr{X}}}
\def\scrY{{\mathscr{Y}}}
\def\scrZ{{\mathscr{Z}}}

\def\scra{{\mathscr a}}
\def\scrb{{\mathscr b}}
\def\scrc{{\mathscr c}}
\def\scrd{{\mathscr d}}
\def\scre{{\mathscr e}}
\def\scrf{{\mathscr f}}
\def\scrg{{\mathscr g}}
\def\scrh{{\mathscr h}}
\def\scri{{\mathscr i}}
\def\scrj{{\mathscr j}}
\def\scrk{{\mathscr k}}
\def\scrl{{\mathscr l}}
\def\scrm{{\mathscr m}}
\def\scrn{{\mathscr n}}
\def\scro{{\mathscr o}}
\def\scrp{{\mathscr p}}
\def\scrq{{\mathscr q}}
\def\scrr{{\mathscr r}}
\def\scrs{{\mathscr s}}
\def\scrt{{\mathscr t}}
\def\scru{{\mathscr u}}
\def\scrv{{\mathscr v}}
\def\scrw{{\mathscr w}}
\def\scrx{{\mathscr x}}
\def\scry{{\mathscr y}}
\def\scrz{{\mathscr z}}


%%% TT font

\def\ttA{{\mathtt{A}}}
\def\ttB{{\mathtt{B}}}
\def\ttC{{\mathtt{C}}}
\def\ttD{{\mathtt{D}}}
\def\ttE{{\mathtt{E}}}
\def\ttF{{\mathtt{F}}}
\def\ttG{{\mathtt{G}}}
\def\ttH{{\mathtt{H}}}
\def\ttI{{\mathtt{I}}}
\def\ttJ{{\mathtt{J}}}
\def\ttK{{\mathtt{K}}}
\def\ttL{{\mathtt{L}}}
\def\ttM{{\mathtt{M}}}
\def\ttN{{\mathtt{N}}}
\def\ttO{{\mathtt{O}}}
\def\ttP{{\mathtt{P}}}
\def\ttQ{{\mathtt{Q}}}
\def\ttR{{\mathtt{R}}}
\def\ttS{{\mathtt{S}}}
\def\ttT{{\mathtt{T}}}
\def\ttU{{\mathtt{U}}}
\def\ttV{{\mathtt{V}}}
\def\ttW{{\mathtt{W}}}
\def\ttX{{\mathtt{X}}}
\def\ttY{{\mathtt{Y}}}
\def\ttZ{{\mathtt{Z}}}

\def\tta{{\mathtt a}}
\def\ttb{{\mathtt b}}
\def\ttc{{\mathtt c}}
\def\ttd{{\mathtt d}}
\def\tte{{\mathtt e}}
\def\ttf{{\mathtt f}}
\def\ttg{{\mathtt g}}
\def\tth{{\mathtt h}}
\def\tti{{\mathtt i}}
\def\ttj{{\mathtt j}}
\def\ttk{{\mathtt k}}
\def\ttl{{\mathtt l}}
\def\ttm{{\mathtt m}}
\def\ttn{{\mathtt n}}
\def\tto{{\mathtt o}}
\def\ttp{{\mathtt p}}
\def\ttq{{\mathtt q}}
\def\ttr{{\mathtt r}}
\def\tts{{\mathtt s}}
\def\ttt{{\mathtt t}}
\def\ttu{{\mathtt u}}
\def\ttv{{\mathtt v}}
\def\ttw{{\mathtt w}}
\def\ttx{{\mathtt x}}
\def\tty{{\mathtt y}}
\def\ttz{{\mathtt z}}







%% serif fonts

\def\sfA{{\sf A}}
\def\sfB{{\sf B}}
\def\sfC{{\sf C}}
\def\sfD{{\sf D}}
\def\sfE{{\sf E}}
\def\sfF{{\sf F}}
\def\sfG{{\sf G}}
\def\sfH{{\sf H}}
\def\sfI{{\sf I}}
\def\sfJ{{\sf J}}
\def\sfK{{\sf K}}
\def\sfL{{\sf L}}
\def\sfM{{\sf M}}
\def\sfN{{\sf N}}
\def\sfO{{\sf O}}
\def\sfP{{\sf P}}
\def\sfQ{{\sf Q}}
\def\sfR{{\sf R}}
\def\sfS{{\sf S}}
\def\sfT{{\sf T}}
\def\sfU{{\sf U}}
\def\sfV{{\sf V}}
\def\sfW{{\sf W}}
\def\sfX{{\sf X}}
\def\sfY{{\sf Y}}
\def\sfZ{{\sf Z}}

\def\sfa{{\sf a}}
\def\sfb{{\sf b}}
\def\sfc{{\sf c}}
\def\sfd{{\sf d}}
\def\sfe{{\sf e}}
\def\sff{{\sf f}}
\def\sfg{{\sf g}}
\def\sfh{{\sf h}}
\def\sfi{{\sf i}}
\def\sfj{{\sf j}}
\def\sfk{{\sf k}}
\def\sfl{{\sf l}}
\def\sfm{{\sf m}}
\def\sfn{{\sf n}}
\def\sfo{{\sf o}}
\def\sfp{{\sf p}}
\def\sfq{{\sf q}}
\def\sfr{{\sf r}}
\def\sfs{{\sf s}}
\def\sft{{\sf t}}
\def\sfu{{\sf u}}
\def\sfv{{\sf v}}
\def\sfw{{\sf w}}
\def\sfx{{\sf x}}
\def\sfy{{\sf y}}
\def\sfz{{\sf z}}









\def\bfmath#1{{\mathchoice{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$\scriptstyle#1$}}%
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}



%boldmath

%%%


\def\bfma{\bfmath{a}}
\def\bfmb{\bfmath{b}}
\def\bfmd{\bfmath{d}}
\def\bfme{\bfmath{e}}
\def\bfmm{\bfmath{m}}
\def\bfmq{\bfmath{q}}
\def\bfmr{\bfmath{r}}
\def\bfmv{\bfmath{v}}
\def\bfmx{\bfmath{x}}
\def\bfmy{\bfmath{y}}
\def\bfmu{\bfmath{u}}
\def\bfmw{\bfmath{w}}


\def\bfmhaw{\bfmath{\haw}}

\def\bfmz{\bfmath{z}}

\def\bfmA{\bfmath{A}}
\def\bfmB{\bfmath{B}}

\def\bfmC{\bfmath{C}}
\def\bfmD{\bfmath{D}}
\def\bfmE{\bfmath{E}}
\def\bfmF{\bfmath{F}}
\def\bfmG{\bfmath{G}}
\def\bfmH{\bfmath{H}}
\def\bfmI{\bfmath{I}}
\def\bfmhaI{\bfmath{\haI}}
\def\bfmhaL{\bfmath{\haL}}
\def\bfmL{\bfmath{L}}
\def\bfmM{\bfmath{M}}
\def\bfmN{\bfmath{N}}
\def\bfmQ{\bfmath{Q}}
\def\bfmR{\bfmath{R}}
\def\bfmbarR{\bfmath{\bar{R}}}





\def\bfmS{\bfmath{S}}
\def\bfmT{\bfmath{T}}
\def\bfmU{\bfmath{U}}


\def\bfmhaN{\bfmath{\widehat N}}
\def\bfmhaQ{\bfmath{\widehat Q}}

\def\bfmX{\bfmath{X}}
\def\bfmtilX{\bfmath{\widetilde{X}}}

\def\bfmtilQ{\bfmath{\widetilde{Q}}}

\def\bfmtilq{\tilde{\bfmath{q}}}


%\def\bfmtilX{\tilde \bfmX}


\def\bfmY{\bfmath{Y}}
\def\bfmhaY{\bfmath{\widehat Y}}


\def\bfmhhaY{\bfmath{\hhaY}} %\widehat{\widehat{Y}}}}
\def\bfmhhaY{\hbox to 0pt{$\widehat{\bfmY}$\hss}\widehat{\phantom{\raise 1.25pt\hbox{$\bfmY$}}}}


\def\bfmV{\bfmath{V}}
\def\bfmW{\bfmath{W}}
\def\bfmhaW{\bfmath{\haW}}
\def\bfmZ{\bfmath{Z}}


\def\bfmhaZ{{\bfmath{\widehat Z}}}


%\def\bfmhaq{\bfmath{\widehat q}}
\def\bfmhaw{\bfmath{\widehat w}}
\def\bfmhay{\bfmath{\widehat y}}
\def\bfmhaz{\bfmath{\widehat z}}
\def\bfmhaQ{\bfmath{\widehat Q}}
\def\bfmhaS{\bfmath{\widehat S}}
\def\bfmhaU{\bfmath{\widehat U}}
\def\bfmhaW{\bfmath{\widehat W}}






\def\bfatom{\bfmath{\theta}}
\def\bfPhi{\bfmath{\Phi}}


\def\bfeta{\bfmath{\eta}}

\def\bfpi{\bfmath{\pi}}



\def\bfphi{\bfmath{\phi}}
\def\bfpsi{\bfmath{\psi}}


\def\bfrho{\bfmath{\rho}}
\def\bfzeta{\bfmath{\zeta}}

\def\bfUpsilon{\bfmath{\Upsilon}}





% \ha prefixes

%  Wide hat

\def\haPsi{{\widehat{\Psi}}}
\def\haGamma{{\widehat{\Gamma}}}
\def\haSigma{{\widehat{\Sigma}}}
\def\habfPhi{{\widehat{\bfPhi}}}
\def\haP{{\widehat P}}




%  Hat

\def\hac{{\hat c}}
\def\haz{\hat{z}}
\def\hai{{\hat {\i}}}
\def\haf{{\hat f}}
\def\hag{{\hat g}}
\def\ham{{\hat m}}
\def\hah{{\hat h}}
\def\hap{{\hat p}}
\def\haq{{\hat q}}

%\def\bfmhaq{{\bfmath{$\hat q$}}}

\def\bfmhaQ{{\bfmath{$\widehat Q$}}}

\def\hav{\hat v}
\def\haw{{\hat w}}
\def\hay{{\hat y}}


\def\haF{{\widehat F}}
\def\haI{{\hat I}}
\def\haJ{{\hat J}}

\def\haN{\hat{N}}

\def\haQ{{\widehat Q}}
\def\haT{{\widehat T}}
\def\haW{{\widehat W}}

\def\haeta{{\hat\eta}}

\def\hatheta{{\hat\theta}}
\def\hapsi{{\hat\psi}}
\def\hapi{{\hat\pi}}
\def\hanu{{\hat\nu}}
\def\hamu{{\hat\mu}}
\def\halpha{{\hat\alpha}}
\def\habeta{{\hat\beta}}
\def\hagamma{{\hat\gamma}}

\def\halambda{{\hat\lambda}}
\def\haLambda{{\hat\Lambda}}

% \rm prefixes

\def\rmA{{\rm A}}
\def\rmB{{\rm B}}
\def\rmC{{\rm C}}
\def\rmD{{\rm C}}
\def\rmE{{\rm E}}
\def\rmH{{\rm H}}
\def\rmI{{\rm I}}
\def\rmM{{\rm M}}
\def\rmP{{\rm P}}
\def\rmQ{{\rm Q}}

\def\rmd{{\rm d}}
\def\rmg{{\rm g}}
\def\rmk{{\rm k}}
\def\rmu{{\rm u}}
\def\rmx{{\rm x}}

\def\rmP{{\rm P}}
\def\rmE{{\rm E}}




% \til prefixes

% Wide tilde

\def\til={{\widetilde =}}
\def\tilPhi{{\widetilde \Phi}}
\def\tilN{{\widetilde N}}
\def\tilP{{\widetilde P}}
\def\tilQ{{\widetilde Q}}
\def\tilT{\widetilde T}
\def\tilW{\widetilde W}




% Tilde

\def\tilmu{{\tilde \mu}}
\def\tilpi{{\tilde \pi}}
\def\tilbfX{{\bf\tilde X}}
\def\tilbfm{{\bf \tilde  m}}
\def\tiltheta{{\tilde \theta}}
\def\tile{\tilde e}
\def\tilsigma{\tilde \sigma}
\def\tiltau{\tilde \tau}




%Caligraphy

\def\clA{{\cal A}}
\def\clB{{\cal B}}
\def\clC{{\cal C}}
\def\clD{{\cal D}}
\def\clE{{\cal E}}
\def\clF{{\cal F}}
\def\clG{{\cal G}}
\def\clH{{\cal H}}
\def\clJ{{\cal J}}
\def\clI{{\cal I}}
\def\clK{{\cal K}}
\def\clL{{\cal L}}
\def\clM{{\cal M}}
\def\clN{{\cal N}}
\def\clO{{\cal O}}
\def\clP{{\cal P}}
\def\clQ{{\cal Q}}
\def\clR{{\cal R}}
\def\clS{{\cal S}}
\def\clT{{\cal T}}
\def\clU{{\cal U}}
\def\clV{{\cal V}}
\def\clW{{\cal W}}
\def\clX{{\cal X}}
\def\clY{{\cal Y}}
\def\clZ{{\cal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISCELLANEOUS


%%%%%%%% Changed the defn of atom on 5/25.  What do you think?


\def\bfatom{{\mbox{\boldmath$\alpha$}}}
\def\atom{{\mathchoice{\bfatom}{\bfatom}{\alpha}{\alpha}}}

\def\Gexp{\clG^+(\gamma)}
\def\Gexps{\clG^+(s)}

%\def\Var{\hbox{\rm Var}\,}

%\def\Var{{\text{Var}}}
\def\Var{{\mathbb{V}\sfa \sfr}}


\def\At{A_+}
\def\barAt#1{\overline{A_+(#1)}}

\def\head#1{\subsubsection*{#1}}



%%\genfrac{}{}{}{1}{1}{2} The \genfrac command is valid only in math mode.
%It takes six arguments, say L, R, w, s, N, D. The translation is a fraction N over D,
% with left and right delimiters L and R. The parameter w specifies  the width of the
%  fraction rule. It can be omitted. The parameter s specifies the style, it is a number
%  between 0 and 3, interpreted as  \displaystyle, \textstyle, scriptstyle  \scriptscriptstyle.
%  It can be empty.

\def\atopss#1#2{\genfrac{}{}{0cm}{2}{#1}{#2}}

\def\atop#1#2{\genfrac{}{}{0pt}{}{#1}{#2}}


 \def\FRAC#1#2#3{\genfrac{}{}{}{#1}{#2}{#3}}



\def\fraction#1#2{{\mathchoice{\FRAC{0}{#1}{#2}}%
{\FRAC{1}{#1}{#2}}%
{\FRAC{3}{#1}{#2}}%
{\FRAC{3}{#1}{#2}}}}

\def\ddt{{\mathchoice{\FRAC{1}{d}{dt}}%
{\FRAC{1}{d}{dt}}%
{\FRAC{3}{d}{dt}}%
{\FRAC{3}{d}{dt}}}}


\def\ddr{{\mathchoice{\FRAC{1}{d}{dr}}%
{\FRAC{1}{d}{dr}}%
{\FRAC{3}{d}{dr}}%
{\FRAC{3}{d}{dr}}}}


\def\ddr{{\mathchoice{\FRAC{1}{d}{dy}}%
{\FRAC{1}{d}{dy}}%
{\FRAC{3}{d}{dy}}%
{\FRAC{3}{d}{dy}}}}


\def\ddtp{{\mathchoice{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{1}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}%
{\FRAC{3}{d^{\hbox to 2pt{\rm\tiny +\hss}}}{dt}}}}


\def\ddalpha{{\mathchoice{\FRAC{1}{d}{d\alpha}}%
{\FRAC{1}{d}{d\alpha}}%
{\FRAC{3}{d}{d\alpha}}%
{\FRAC{3}{d}{d\alpha}}}}



\def\half{{\mathchoice{\FRAC{1}{1}{2}}%
{\FRAC{1}{1}{2}}%
{\FRAC{3}{1}{2}}%
{\FRAC{3}{1}{2}}}}

\def\third{{\mathchoice{\FRAC{1}{1}{3}}%
{\FRAC{1}{1}{3}}%
{\FRAC{3}{1}{3}}%
{\FRAC{3}{1}{3}}}}

\def\fourth{{\mathchoice{\FRAC{1}{1}{4}}%
{\FRAC{1}{1}{4}}%
{\FRAC{3}{1}{4}}%
{\FRAC{3}{1}{4}}}}

 \def\threefourth{{\mathchoice{\FRAC{1}{3}{4}}%
{\FRAC{1}{3}{4}}%
{\FRAC{3}{3}{4}}%
{\FRAC{3}{3}{4}}}}

\def\sixth{{\mathchoice{\FRAC{1}{1}{6}}%
{\FRAC{1}{1}{6}}%
{\FRAC{3}{1}{6}}%
{\FRAC{3}{1}{6}}}}

\def\eighth{{\mathchoice{\FRAC{1}{1}{8}}%
{\FRAC{1}{1}{8}}%
{\FRAC{3}{1}{8}}%
{\FRAC{3}{1}{8}}}}



\def\eqdist{\buildrel{\rm dist}\over =}

\def\eqdef{\mathbin{:=}}

\def\lebmeas{\mu^{\hbox{\rm \tiny Leb}}}
\def\Prbty{{\cal  M}}



\def\Prob{{\sf P}}
\def\Probsub{{\sf P\! }}
\def\Expect{{\sf E}}

\def\taboo#1{{{}_{#1}P}}

\def\io{{\rm i.o.}}


\def\as{{\rm a.s.}}
\def\Vec{{\rm vec\, }}

%\def\eq#1/{(\ref{#1})}

\def\oneN{{\displaystyle\frac{1}{ N}}}

\def\average#1,#2,{{1\over #2} \sum_{#1}^{#2}}

\def\enters{\hbox{ \rm \  enters\  }}

\def\eye(#1){{\bf(#1)}\quad}
\def\epsy{\varepsilon}

\def\varble{\,\cdot\,}

\def\var{{\bV\sfa\sfr}}
%%%%%%%%%%THEOREMS and EQUATIONS


%\newtheorem{theorem}{{\bf Theorem}}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{{\bf Definition}}
%\newtheorem{remark}{{\bf Remark}}
%\newtheorem{proposition}{{\bf Proposition}}
%\newtheorem{lemma}{{\bf Lemma}}



\def\Lemma#1{Lemma~\ref{t:#1}}
\def\Proposition#1{Proposition~\ref{t:#1}}
\def\Theorem#1{Theorem~\ref{t:#1}}
\def\Corollary#1{Corollary~\ref{t:#1}}
\def\Remark#1{Remark~\ref{t:#1}}


\def\Section#1{Section~\ref{#1}}

\def\Figure#1{Figure~\ref{f:#1}}
\def\Chapter#1{Chapter~\ref{c:#1}}

\def\Appendix#1{Appendix~\ref{c:#1}}

\def\eq#1/{(\ref{e:#1})}

%\newcommand{\inp}[2]{{\langle #1, #2 \rangle}}
%\newcommand{\inpr}[2]{{\langle #1, #2 \rangle}_\bR}



\newcommand{\beqn}[1]{\notes{#1}%
\begin{eqnarray} \elabel{#1}}

\newcommand{\eeqn}{\end{eqnarray} }


\newcommand{\beq}[1]{\notes{#1}%
\begin{equation}\elabel{#1}}

\newcommand{\eeq}{\end{equation}}

\def\bdes{\begin{description}}
\def\edes{\end{description}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%  \bar prefixes (improved?)
\def\bara{{\overline {a}}}

\def\barc{{\overline {c}}}

\def\barf{{\overline {f}}}
\def\barg{{\overline {g}}}
\def\barh{{\overline {h}}}
\def\barI{{\overline {l}}}
\def\barm{{\overline {m}}}
\def\barn{{\overline {n}}}

\def\barp{{\overline {p}}}
\newcommand{\barx}{{\bar{x}}}
\def\bary{{\overline {y}}}
\def\barA{{\overline {A}}}
\def\barB{{\overline {B}}}
\def\barC{{\overline {C}}}
\def\barE{{\overline {E}}}
\def\barM{{\overline {M}}}
\def\barP{{\overline {P}}}
\def\barQ{{\overline {Q}}}
\def\barT{{\overline {T}}}


\def\undern{{\underline{n}}}
\def\ubarho{{\underline{\rho}}}

\def\baratom{{\overline{\atom}}}
\def\barho{{\overline{\rho}}}
\def\barmu{{\overline{\mu}}}
\def\barnu{{\overline{\nu}}}
\def\baralpha{{\overline{\alpha}}}
\def\barbeta{{\overline{\beta}}}

\def\baralpha{{\overline{\alpha}}}
\def\bareta{{\overline{\eta}}}



\def\barbP{\overline{\bfPhi}}
\def\barPhi{\overline{\Phi}}
\def\barF{\overline{\clF}}
\def\barsigma{\overline{\sigma}}

\def\barSigma{\overline{\Sigma}}


\def\bartau{\overline{\tau}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOR SAMPLED CHAINS IN CH{CRITERIA}

\def\Sampsigma{\hat{\sigma}}
\def\Samptau{\hat{\tau}}
\def\SampP{\hat{P}}
\def\SampPhi{\hat{\Phi}}
\def\SampbfPhi{\hat{\bfPhi}}
\def\SampF{\hat{\cal F}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% LIST

%\newcounter{rmnum}
%\newenvironment{romannum}{\begin{list}{{\upshape (\roman{rmnum})}}{\usecounter{rmnum}
%\setlength{\leftmargin}{24pt}
%\setlength{\rightmargin}{16pt}
%\setlength{\itemindent}{-1pt}
%}}{\end{list}}
%
%\newcounter{anum}
%\newenvironment{alphanum}{\begin{list}{{\upshape (\alph{anum})}}{\usecounter{anum}
%\setlength{\leftmargin}{24pt}
%\setlength{\rightmargin}{16pt}
%\setlength{\itemindent}{-1pt}
%}}{\end{list}}




\newcounter{rmnum}
\newenvironment{romannum}{\begin{list}{{\upshape (\roman{rmnum})}}{\usecounter{rmnum}
\setlength{\leftmargin}{14pt}
\setlength{\rightmargin}{8pt}
\setlength{\itemindent}{-1pt}
}}{\end{list}}

\newcounter{anum}
\newenvironment{alphanum}{\begin{list}{{\upshape (\alph{anum})}}{\usecounter{anum}
\setlength{\leftmargin}{14pt}
\setlength{\rightmargin}{8pt}
\setlength{\itemindent}{-1pt}
}}{\end{list}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASSUMPTIONS



\newenvironment{assumptions}[1]{%
\setcounter{keep_counter}{\value{#1}}
\def\aref{#1}
\begin{list}{\sf\, (#1\arabic{#1})\mindex{Assumption (#1\arabic{#1})}\, }{\usecounter{#1}%
\setlength{\rightmargin}{\leftmargin}}
\setcounter{#1}{\value{keep_counter}}}%
{\end{list}}



\def\ass(#1:#2){(#1\ref{#1:#2})}




\def\ritem#1{
\item[{\sf \ass(\current_model:#1)}]
}

\newenvironment{recall-ass}[1]{%
\begin{description}
\def\current_model{#1}}{
\end{description}
}


\def\Ebox#1#2{%
\begin{center}
 \parbox{#1\hsize}{\epsfxsize=\hsize \epsfbox{#2}}
\end{center}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Tweedie

%\newcommand{\bd}{\begin{description}}
%\newcommand{\ed}{\end{description}}
%\newcommand{\bt}{\begin{theorem}}
%\newcommand{\et}{\end{theorem}}
%\newcommand{\ba}{\begin{array}{rcl}}
%\newcommand{\ea}{\end{array}}


\def\MT{\cite{meytwe92d}}

